Source Coding Based Millimeter-Wave Channel Estimation with Deep Learning Based Decoding

The speed at which millimeter-Wave (mmWave) channel estimation can be carried out is critical for the adoption of mmWave technologies. This is particularly crucial because mmWave transceivers are equipped with large antenna arrays to combat severe path losses, which consequently creates large channel matrices, whose estimation may incur significant overhead. This paper focuses on the mmWave channel estimation problem. Our objective is to reduce the number of measurements required to reliably estimate the channel. Specifically, channel estimation is posed as a "source compression" problem in which measurements mimic an encoded (compressed) version of the channel. Decoding the observed measurements, a task which is traditionally computationally intensive, is performed using a deep-learning-based approach, facilitating a high-performance channel discovery. Our solution not only outperforms state-of-the-art compressed sensing methods, but it also determines the lower bound on the number of measurements required for reliable channel discovery.

==> beamDiscovery.tex <==
Introduction .... 


Explain the details of how a linear source coding algorithm could be applied for non-adaptive mm-wave beam discovery.

Start with a simple $n_r \times 1$ channel. Then, generalize to arbitrary $n_r \times n_t$ channels in the last subsection.


\subsection{Measurements Design}

Explain the design of tx-precoders and rx-combiners.



\subsection{Sufficient Statistic}

Prove that the resultant $\boldsymbol{Y^s}$ channel measurement matrix is sufficient to be mapped to a unique channel matrix $\boldsymbol{Q^a}$.

\subsection{Mapping Function}

Explain how to map $\boldsymbol{Y^s} \Longrightarrow \boldsymbol{Q^a}$.

\subsection{Multiple TX and RX Antennas}

Generalize to multiple TX and multiple RX antenna arrays.

Simplify the procedure compared to what we had in INFOCOM paper.

If possible, provide an illustrative picture/diagram to ease explanation.

==> problemStatement.tex <==
We cast the channel estimation problem as a beam discovery problem. That is, we seek to find the path gain values of the strong paths between TX and RX and their respective transmit and receive angular directions.
Towards this objective, we strive to directly obtain $\boldsymbol{Q^a}$ rather than\footnote{Recall that $\boldsymbol{Q} = \boldsymbol{U_r}\boldsymbol{Q^a} \boldsymbol{U}_{\boldsymbol{t}}^H$. Also see Eq. (\ref{eqn:Qa_from_Q}).} $\boldsymbol{Q}$.

Recall that according to the channel sparsity assumption, only $n_p \ll n_r, n_t$ non-zero components exist in $\boldsymbol{Q^a}$.
Sparsity is one form of data structures that are known to be compressible.
Hence, channel matrices $\boldsymbol{Q^a}$ of size $n_r {\times} n_t$ can be efficiently represented using smaller matrices $\boldsymbol{Y^s}$ of size $m_r {\times} m_t$ where $m_r < n_r$ and $m_t < n_t$.
\textbf{Our objective is to find a channel measurement algorithm that is based on \textit{linear} source codes to obtain such $\boldsymbol{Y^s}$ matrices}.
Then, we estimate $\boldsymbol{Q^a}$ using a mapping function $\xi : \boldsymbol{Y^s} \longrightarrow \hat{\boldsymbol{Q}}^{\boldsymbol{a}}$.
Note that we focus on finding error-free $\boldsymbol{Y^s}$ matrices whose entries are $y^s_{i,j}$ are obtained using the tx-precoder $\boldsymbol{f}_j$ and rx-combiner $\boldsymbol{w}_i$ (see Eq. (\ref{eqn:error-free_symbols})).

Our design variables are the tx-precoding vectors $\boldsymbol{f}_j$, the rx-combining vectors $\boldsymbol{w}_i$ and the mapping function $\xi(\cdot)$. Note that the design of $\boldsymbol{f}_j$ and $\boldsymbol{w}_i$ are dictated by the linear source coding algorithm. Hence, we might as well consider the choice of the source coding algorithm as a design variable.

